Achieving Real-Time LiDAR 3D Object Detection on a Mobile Device

3D object detection is an important task, especially in the autonomous driving application domain. However, it is challenging to support the real-time performance with the limited computation and memory resources on edge-computing devices in self-driving cars. To achieve this, we propose a compiler-aware unified framework incorporating network enhancement and pruning search with the reinforcement learning techniques, to enable real-time inference of 3D object detection on the resource-limited edge-computing devices. Specifically, a generator Recurrent Neural Network (RNN) is employed to provide the unified scheme for both network enhancement and pruning search automatically, without human expertise and assistance. And the evaluated performance of the unified schemes can be fed back to train the generator RNN. The experimental results demonstrate that the proposed framework firstly achieves real-time 3D object detection on mobile devices (Samsung Galaxy S20 phone) with competitive detection performance.

==> macros.tex <==


\newcommand*\circledgray[1]{% require `tikz`
	\tikz[baseline=(char.base)]{\node[
        shape=circle, draw=none,  thick, 
        fill=gray!40,inner sep=0.6pt] (char) 
    {\textcolor{black}{\sffamily#1}}; 
}}


% \newcommand*\circled[1]{\tikz[baseline=(char.base)]{
%   \node[shape=circle,draw,fill=black,text=white,font=\bf,inner sep=0.5pt] (char)
%   {\scriptsize#1};
% }}

\newcommand*\circledwhite[1]{\tikz[baseline=(char.base)]{
  \node[shape=circle,draw,fill=white,text=black,font=\bf,inner sep=0.5pt] (char)
  {\scriptsize#1};
}}

\newcommand*\circled[1]{\tikz[baseline=(char.base)]{\node[shape=circle,draw,inner sep=0.6pt] (char) {#1};}}

% \newcommand{\etal}{\textit{et al.}}

% \newcommand{\putsec}[2]{\vspace{-0.1in}\section{#2}\label{sec:#1}\vspace{-0.05in}}
% \newcommand{\putssec}[2]{\vspace{-0.0in}\subsection{#2}\label{ssec:#1}\vspace{-0.0in}}
% \newcommand{\putsssec}[2]{\vspace{-0.0in}\subsubsection{#2}\label{sssec:#1}\vspace{-0.0in}}
% %\newcommand{\putsssecX}[1]{\vspace{0.0in}\subsubsection*{#1}\vspace{0.0in}}
% \newcommand{\putsssecX}[1]{\vspace{0.0in}\noindent\textbf{#1:}}

% \newcommand{\figref}[1]{Figure~\ref{fig:#1}}
% \newcommand{\eqnref}[1]{Equation~\ref{eq:#1}}
% \newcommand{\tabref}[1]{Table~\ref{tab:#1}}
% \newcommand{\secref}[1]{Section~\ref{sec:#1}}
% \newcommand{\ssecref}[1]{Section~\ref{ssec:#1}}
% \newcommand{\sssecref}[1]{Section~\ref{sssec:#1}}


\newcommand{\squishlist}{
    \begin{list}{$\bullet$}
        { \setlength{\itemsep}{0pt}      \setlength{\parsep}{0pt}
            \setlength{\topsep}{0.5pt}       \setlength{\partopsep}{0pt}
            \setlength{\listparindent}{-2pt}
            \setlength{\itemindent}{-5pt}
            \setlength{\leftmargin}{0.5em} \setlength{\labelwidth}{0em}
            \setlength{\labelsep}{0.2em} } }
    
\newcommand{\squishend}{
\end{list}  }


\newcommand{\COMMENT}[1]{#1}
\newcommand{\xulong}[1]{\COMMENT{\textcolor{brown}{\sf\bfseries Xulong: #1}}}
\newcommand{\GY}[1]{\COMMENT{\textcolor{orange}{\bfseries Geng: #1}}}
\newcommand{\yx}[1]{\COMMENT{\textcolor{cyan}{\sf\bfseries Yuxuan: #1}}}
\newcommand{\jia}[1]{\COMMENT{\textcolor{blue}{\sf\bfseries Hongjia: #1}}}
\newcommand{\todo}[1]{\COMMENT{{\color{red} #1}}}

\newcommand{\added}[1]{\COMMENT{{\color{blue} #1}}}

% Uncomment this to remove the inline comments
%   \renewcommand{\COMMENT}[1]{}

\newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}  

